Electricity Theft Detection using Machine Learning

Non-technical losses (NTL) in electric power grids arise through electricity theft, broken electric meters or billing errors. They can harm the power supplier as well as the whole economy of a country through losses of up to 40% of the total power distribution. For NTL detection, researchers use artificial intelligence to analyse data. This work is about improving the extraction of more meaningful features from a data set. With these features, the prediction quality will increase.

==> discussion.tex <==
\section{Discussion}
This work shows that the newly extracted features from the data lead to a better prediction quality than the former daily average features. The AUC with the combination of all the features gained is just slightly better than the AUC of the daily average features. A quite important cause for this behaviour is that the provided data set is a real world data set, which contains noise, outliers, or even errors in the data through input error. \todo{syntax} However, even a small improvement in the NTL detection would cause to a reduction of the cost for carrying out inspections for the customers. Furthermore, the energy company would be able to increase the stability of the electrical power grid by decreasing the NTL cases. Also, the partner company of this project would have the benefit of raising their equity through the improvement of their products. \\
Surprisingly, the gradient boosted tree always delivered poor classification results. Contrarily, in other papers the classifier showed good prediction quality~\cite{roe2005boosted, chen2016xgboost}. This could be explained with the ``no free lunch'' (NFL) theorem, which points out that the best machine learning model does not exist~\cite{wolpert1996lack}.
